MAZE: Data-Free Model Stealing Attack Using Zeroth-Order Gradient Estimation

Model Stealing (MS) attacks allow an adversary with black-box access to a Machine Learning model to replicate its functionality, compromising the confidentiality of the model. Such attacks train a clone model by using the predictions of the target model for different inputs. The effectiveness of such attacks relies heavily on the availability of data necessary to query the target model. Existing attacks either assume partial access to the dataset of the target model or availability of an alternate dataset with semantic similarities. This paper proposes MAZE -- a data-free model stealing attack using zeroth-order gradient estimation. In contrast to prior works, MAZE does not require any data and instead creates synthetic data using a generative model. Inspired by recent works in data-free Knowledge Distillation (KD), we train the generative model using a disagreement objective to produce inputs that maximize disagreement between the clone and the target model. However, unlike the white-box setting of KD, where the gradient information is available, training a generator for model stealing requires performing black-box optimization, as it involves accessing the target model under attack. MAZE relies on zeroth-order gradient estimation to perform this optimization and enables a highly accurate MS attack. Our evaluation with four datasets shows that MAZE provides a normalized clone accuracy in the range of 0.91x to 0.99x, and outperforms even the recent attacks that rely on partial data (JBDA, clone accuracy 0.13x to 0.69x) and surrogate data (KnockoffNets, clone accuracy 0.52x to 0.97x). We also study an extension of MAZE in the partial-data setting and develop MAZE-PD, which generates synthetic data closer to the target distribution. MAZE-PD further improves the clone accuracy (0.97x to 1.0x) and reduces the query required for the attack by 2x-24x.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> data-free-kd.tex <==
\textbf{Adversarial Belief Matching (ABM)~\cite{abm}:} ABM performs knowledge distillation by using images generated from a generative model $G(z; \phi)$. This generative model is trained to produce inputs $x$ such that the predictions of the teacher model $T(X;\theta_T)$ and the predictions of the student model $S(x;\theta_S)$ are dissimilar. Specifically, $G$ is trained to maximize the KL-divergence between the predictions of the teacher and student model using the loss function shown in  Eqn.~\ref{eq:abm_g}. The student model on the other hand is trained to match the predictions of the teacher by minimizing the KL-divergence between the predictions of $T$ and $S$ using the loss function in Eqn. ~\ref{eq:abm_s}. By iteratively updating the generator and student model, ABM performs KD between $T$ and $S$.

\begin{align} 
x &= G(z) \\
\mathcal{L}_G &= - D_{K L}\left(T\left(\boldsymbol{x}\right) \|\ S\left(\boldsymbol{x}\right)\right) \label{eq:abm_g}\\
\mathcal{L}_S &= D_{K L}\left(T\left(\boldsymbol{x}\right) \|\ S\left(\boldsymbol{x}\right)\right)\label{eq:abm_s}
\end{align}

In addition to the basic idea presented above, ABM also uses an additional Attention Transfer ~\cite{at} term in the loss function of the student. AT tries to match the attention maps of the intermediate activations between the student and teacher networks which helps in KD. 

We note that the training process of the student model in ABM assumes white-box access to the target model as the loss terms of both the student and the generator models (Eqn.~\ref{eq:abm_g},~\ref{eq:abm_s}) involve back propagating through the target model $T$. Moreover, ABM also uses AT, which requires access to the intermediate activations of $T$. Due to these requirements, ABM cannot be directly used to perform model stealing as we only have black-box access to the target model. However, in the following section we show how zeroth order optimization along with training objectives similar to ABM can be used to develop our MS attack.



\textbf{Dreaming To Distill (DTD)~\cite{dreaming}:} Given a DNN model $T$ and a target class $y$, DTD proposes to use the loss function of $T$ along with various image-prior terms to generate realistic images which resemble the images from the target class in the training distribution of $T$. DTD leverages the observation that natural images tend to have low variance and l2-norm and uses this to craft realistic inputs. For instance, given a randomly initialized input $x$ and a target class $y$, one could potentially synthesis an image from the target class by framing it as an optimization problem using the loss function $\mathcal{L}$ of a DNN and additional regularization terms as shown in Eqn.~\ref{eq:dream_prior}
\begin{align}
\min _{x} \mathcal{L}(T(x), y))+\mathcal{R}_p(x)\label{eq:dream_prior}
\end{align}
 In this equation, $\mathcal{R}_p$ is the image prior regularization term which steers $x$ away from unnatural images. The key insight of DTD is that the statistics of the batch norm layers (channel-wise mean and variance information of the activation maps for the training data) can be leveraged to frame the problem of generating realistic images. To this end, DTD proposes \emph{Deep-Inversion}, which uses statistics from the batch-norm layers of the DNN as an added regularization term in Eqn.~\ref{eq:dream_prior} to enable the synthesis of realistic inputs. In the KD setting, the inputs generated using this technique can be used to train a student model $S$ from the predictions of the teacher model $T$. Furthermore, the paper also proposes \emph{Adaptive Deep-Inversion}, a technique to produce a diverse set of inputs by adding an additional loss term that maximizes the dissimilarity between the outputs of $T$ and $S$. 
 
 Note that, much like ABM, DTD also requires white-box access to the target model since the optimization problem in Eqn.~\ref{eq:dream_prior} requires back propagating through the teacher model. Furthermore, this work requires us to know the running mean and variance information stored in the batch norm layer. This information is unavailable in the black-box setting of the model stealing attack.
 
\subsection{ZO Gradient Estimation in Adversarial ML}
Zeroth Order gradient estimation is a commonly used tool for black-box optimization problems where the gradient information is unavailable. In adversarial machine learning, this technique has been used to craft adversarial examples. The goal here is to cause misclassification by adding targeted perturbations to an input. E.g. given an input $x$, that belongs to class $y$ and a target model $T$, we want to find a perturbation $\delta$ such that the perturbed input $x'=x+\delta$ causes a misclassification in the target model such that $T(x')\neq y$.
In black-box settings, several model evasion attacks ~\cite{zoo,autozoom,sign_bits} use a zeroth order approximation of the gradient of $T$'s loss function to iteratively perturb $x$ in order to find an adversarial example $x'$ that results in a misclassification. 
While these attacks use ZO gradient estimation to craft adversarial examples, in this work we use it to perform model stealing attack by training a clone model $C$ that copies the functionality of the target model.

==> problem.tex <==
\section{Problem Statement}
This paper proposes MAZE-- a data-free model stealing attack.
In this section we formally state the objective and constraints of our proposed attack.

\subsection{Objective}

Consider a target model $T(x;\theta_T)$ which performs a classification task with high accuracy on inputs $x$ sampled from a target distribution $\mathbb{P}_{T}$. Our goal is to train a clone model $C$ which replicates the functionality of $T$ and achieves a high accuracy on the classification task as shown by Eqn. ~\ref{eq:adv_obj}

\begin{align} \label{eq:adv_obj}
\max_{\theta_C}\mathop{\mathbb{E}}_{x\sim \mathbb{P}_{T}}[Acc(C(x;\theta_C))]
%where\ x \sim P_D(X)\nonumber 
\end{align}


\subsection{Constraints}

In this work, we assume that the attacker does not know any details about the Target model's architecture or the model parameters $\theta_T$. The attacker is only allowed black-box access to the target model i.e. the attacker can query the target model with any input $x$ and observe its output predictions $y=T(x;\theta_T)$. In the \emph{data-free} setting of our attack, we assume that the attacker does not have access to the dataset $\mathcal{D}_{T}$  used to train the target model or a good way to sample from the target data distribution $\mathbb{P}_{T}$. We also discuss the applicability of our attack in the \emph{partial-data} setting where this constraint is relaxed and the adversary has access to a set of $100$ random training examples sampled from the training dataset of the target model.

